The inviscid limit of third-order linear and nonlinear acoustic equations

We analyze the behavior of third-order in time linear and nonlinear sound waves in thermally relaxing fluids and gases as the sound diffusivity vanishes. The nonlinear acoustic propagation is modeled by the Jordan--Moore--Gibson--Thompson equation both in its Westervelt and in its Kuznetsov-type forms, that is, including quadratic nonlinearities of the type $(u^2)_{tt}$ and $ (u_t^2 + |\nabla u|^2)_t$. As it turns out, sufficiently smooth solutions of these equations converge in the energy norm to the solutions of the corresponding inviscid models at a linear rate. Numerical experiments illustrate our theoretical findings.

==> preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{calligra}
\usepackage{amsfonts,amsmath,amsthm,amssymb}
\usepackage{mathtools}
\usepackage{hyperref}
\usepackage{autonum}
\usepackage{hhline}
\usepackage{array}
\usepackage{diagbox}
\usepackage{tcolorbox}
\usepackage{mdframed}
\usepackage{multicol}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{moreverb}
\usepackage{bbm}
\usepackage[margin=1.4in]{geometry}
\usepackage{todonotes}
\usepackage{scalerel,amssymb}
\allowdisplaybreaks
\usepackage{mathrsfs}  
\usepackage{lineno}
\usepackage{todonotes}
\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{arrows.meta}
\usepackage{siunitx}
\usepackage[numbers,sort&compress]{natbib}
\definecolor{mygreen}{HTML}{43a047}
\usepackage{subcaption}
\usepackage{doi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Letters, Symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\calA{\mathcal{A}}
%\def\ooal{\tfrac{1}{\alpha}}
\def\ooal{\alpha^{-1}}
\def\ulal{\underline{\alpha}}
\def\olal{\overline{\alpha}}
\def\op{\overline{p}}
\def\opsi{\overline{\psi}}
\def\oq{\overline{q}}
\newcommand{\Om}{\Omega}
\newcommand{\D}{\Delta}
\newcommand{\pn}{p^n}
\DeclareMathOperator*{\esssup}{ess\,sup}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Time-differentiation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ut}{u_t}
\newcommand{\utt}{u_{tt}}
\newcommand{\pt}{p_t}
\newcommand{\ptn}{p_t^n}
\newcommand{\ptt}{p_{tt}}
\newcommand{\pttn}{p_{tt}^n}
\newcommand{\ptttn}{p_{ttt}^n}
\newcommand{\pttt}{p_{ttt}}
\newcommand{\ddt}{\frac{\textup{d}}{\textup{d}t}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Intgration-related
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dt}{\, \textup{d} t}
\newcommand{\ds}{\, \textup{d} s }
\newcommand{\dx}{\, \textup{d} x}
\newcommand{\dxs}{\, \textup{d}x\textup{d}s}
\newcommand{\dxt}{\, \textup{d}x\textup{d}t}
\newcommand{\intTO}{\int_0^t \int_{\Omega}}
\newcommand{\intT}{\int_0^t}
\newcommand{\intO}{\int_{\Omega}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Norms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\nLtwo}[1]{\|#1\|_{L^2}}
\newcommand{\nLthree}[1]{\|#1\|_{L^3}}
\newcommand{\nLfour}[1]{\|#1\|_{L^4}}
\newcommand{\nLsix}[1]{\|#1\|_{L^6}}
\newcommand{\nLinf}[1]{\|#1\|_{L^\infty}}
\newcommand{\nHone}[1]{\|#1\|_{H^1}}
\newcommand{\nHtwo}[1]{\|#1\|_{H^2}}
\newcommand{\nLtwoLtwo}[1]{\|#1\|_{L^2 (L^2)}}
\newcommand{\nLtwoLfour}[1]{\|#1\|_{L^2 (L^4)}}
\newcommand{\nLtwoLsix}[1]{\|#1\|_{L^2 (L^6)}}
\newcommand{\nLtwoLinf}[1]{\|#1\|_{L^2 (L^\infty)}}
\newcommand{\nLinfLtwo}[1]{\|#1\|_{L^\infty (L^2)}}
\newcommand{\nLinfLthree}[1]{\|#1\|_{L^\infty (L^3)}}
\newcommand{\nLinfLfour}[1]{\|#1\|_{L^\infty (L^4)}}
\newcommand{\nLinfLinf}[1]{\|#1\|_{L^\infty (L^\infty)}}
\newcommand{\nLinfHone}[1]{\|#1\|_{L^\infty (H^1)}}
\newcommand{\nLinfHtwo}[1]{\|#1\|_{L^\infty (H^2)}}
\newcommand{\nLinfHthree}[1]{\|#1\|_{L^\infty (H^3)}}
\newcommand{\nLtwoHone}[1]{\|#1\|_{L^2 (H^1)}}
\newcommand{\nHoneHone}[1]{\|#1\|_{H^1 (H^1)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Products
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\prodLtwo}[2]{(#1, #2)_{L^2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Sets
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\R}{\mathbb{R}} 
\newcommand{\N}{\mathbb{N}} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Spaces
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Ltwo}{L^2(\Omega)}
\newcommand{\Hone}{H^1(\Omega)}
\newcommand{\Hthree}{H^3(\Omega)}
\newcommand{\Honetwo}{{H_\diamondsuit^2(\Omega)}}
\newcommand{\Honethree}{{H_\diamondsuit^3(\Omega)}}
\newcommand{\Honefour}{{H_\diamondsuit^4(\Omega)}}
\newcommand{\spaceW}{X^{\textup{W}}}
\newcommand{\spaceK}{X^{\textup{K}}}
\newcommand{\LtwoLtwo}{L^2(0,T; L^2(\Omega))}
\newcommand{\LinfLinf}{L^\infty(0,T; L^\infty(\Omega))}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   % Embedding constants
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\CHone}{C_{H^1, L^4}}
\newcommand{\CHonesix}{C_{H^1, L^6}}
\newcommand{\CHtwo}{C_{H^2, L^\infty}}
\newcommand{\CHtwoeight}{C_{H^2, L^8}}
\newcommand{\CPF}{C_{\textup{PF}}}
\newcommand{\Ctr}{C_{\textup{tr}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Theorem enviroments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem*{assumption*}{Assumptions}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\numberwithin{lemma}{section}
\numberwithin{proposition}{section}
\numberwithin{theorem}{section}
\numberwithin{equation}{section}
\makeatletter
\newcommand{\leqnomode}{\tagsleft@true}
\newcommand{\reqnomode}{\tagsleft@false}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Miscellaneous
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\TK}{\mathcal{T}^{\textup{K}}} 
\newcommand{\TW}{\mathcal{T}^{\textup{W}}} 
\newcommand{\MK}{M_{\textup{K}}} 
\newcommand{\RK}{R_{\textup{K}}} 
\newcommand{\qtil}{\tilde{q}} 
\newcommand{\qtiltil}{\eta} 
\newcommand{\qt}{\mu} 


\definecolor{grey}{rgb}{0.5,0.5,0.5}
\newcommand{\abssig}{|\sigma|} 

